Swap distance minimization in SOV languages. Cognitive and mathematical foundations

Distance minimization is a general principle of language. A special case of this principle in the domain of word order is swap distance minimization. This principle predicts that variations from a canonical order that are reached by fewer swaps of adjacent constituents are lest costly and thus more likely. Here we investigate the principle in the context of the triple formed by subject (S), object (O) and verb (V). We introduce the concept of word order rotation as a cognitive underpinning of that prediction. When the canonical order of a language is SOV, the principle predicts SOV < SVO, OSV < VSO, OVS < VOS, in order of increasing cognitive cost. We test the prediction in three flexible order SOV languages: Korean (Koreanic), Malayalam (Dravidian), and Sinhalese (Indo-European). Evidence of swap distance minimization is found in all three languages, but it is weaker in Sinhalese. Swap distance minimization is stronger than a preference for the canonical order in Korean and especially Malayalam.

==> tables/summary_table_Monte_Carlo_unadjusted_p_values.tex <==
Korean & 4.33 & $<10^{-6}$ & 4.8 & $<10^{-6}$ & 2 & $1.7\cdot 10^{-5}$ & 2.33 & $2.8\cdot 10^{-5}$ & -0.47 & 0.869 \\
Malayalam & 2.33 & $3\cdot 10^{-6}$ & 2.4 & $1\cdot 10^{-6}$ & 0.93 & $9.2\cdot 10^{-3}$ & 1.4 & $9.8\cdot 10^{-5}$ & -0.07 & 0.623 \\
Sinhalese & 2.4 & $1.5\cdot 10^{-3}$ & 1.53 & 0.033 & 2.2 & $1.4\cdot 10^{-5}$ & 0.2 & 0.369 & 0.87 & 0.027

